Stable Surface Regularization for Fast Few-Shot NeRF

This paper proposes an algorithm for synthesizing novel views under few-shot setup. The main concept is to develop a stable surface regularization technique called Annealing Signed Distance Function (ASDF), which anneals the surface in a coarse-to-fine manner to accelerate convergence speed. We observe that the Eikonal loss - which is a widely known geometric regularization - requires dense training signal to shape different level-sets of SDF, leading to low-fidelity results under few-shot training. In contrast, the proposed surface regularization successfully reconstructs scenes and produce high-fidelity geometry with stable training. Our method is further accelerated by utilizing grid representation and monocular geometric priors. Finally, the proposed approach is up to 45 times faster than existing few-shot novel view synthesis methods, and it produces comparable results in the ScanNet dataset and NeRF-Real dataset.

==> Tables/table_eval_llff.tex <==
\begin{table*}[!t]{
\centering
\resizebox{\textwidth}{!}{%
% \resizebox{0.80\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc}

\Xhline{2\arrayrulewidth} 

& & NeRF (Time: 23h) & & & DSNeRF (Time: 22h) & & &Ours (Time: \textbf{0.5h)} \\% \cline{2-10}

& PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\

\hline

fern & 20.00 & 0.58 & 0.41 & \textbf{20.60} & \textbf{0.60} & 0.43 & 20.26 & 0.56 & \textbf{0.34}\\
flower & 17.79 & 0.49 & 0.43 & \textbf{21.79} & \textbf{0.62} & 0.35 & 19.27 & 0.51 & \textbf{0.29}\\
fortress & 19.13 & 0.55 & 0.53 & 23.85& 0.66 & 0.35 & \textbf{24.08} & \textbf{0.67} & \textbf{0.18} \\
horns & 17.57 & 0.51 & 0.50 & \textbf{18.86}& \textbf{0.53} & 0.54& 17.85 & 0.50 & \textbf{0.39} \\
leaves & 13.73 & 0.26 & 0.52 & 15.93 & 0.35 & 0.5& \textbf{16.54} & \textbf{0.45} & \textbf{0.32} \\
orchids & 14.79 & 0.34 & 0.45 & \textbf{16.15} & 0.39 & 0.44 & 15.84 & \textbf{0.42} & \textbf{0.27} \\
room & 22.23 & 0.78 & 0.32 & \textbf{24.46} & \textbf{0.86} & \textbf{0.19} & 23.22 & 0.81 & 0.20 \\
trex & 18.34 & \textbf{0.63} & 0.34 & 18.82 & \textbf{0.63}  & 0.39 & \textbf{19.07} & 0.59 & \textbf{0.30} \\

\hline

Avg. & 17.95 & 0.52 & 0.42 & \textbf{20.06} & \textbf{0.58} & 0.40 & 19.51 & 0.56 & \textbf{0.29}\\

\Xhline{2\arrayrulewidth} 

\end{tabular}
}}
\vspace{1mm}
\caption{Quantitative comparison in NeRF-Real Dataset~\cite{mildenhall2019local, mildenhall2021nerf}. The results are the average of 2 views, 5 views, and 10 views following DSNeRF~\cite{deng2022depth}.}
\label{Table:eval_llff}
\vspace{-3mm}
\end{table*}

==> Tables_sup/ablation_loss_b_opt.tex <==
\begin{table}[h]{

\resizebox{\linewidth}{!}{%
\begin{tabular}{c|l|ccccc}
\hline
  \multicolumn{2}{c|}{} & PSNR $\uparrow$& SSIM $\uparrow$ & LPIPS $\downarrow$ & RMSE $\downarrow$\\
\hline
\multicolumn{2}{c|}{Eikonal} & 20.82 & 0.610 & 0.391 & 0.226\\
\hline
\multirow{4}{*}{Ours}& $b_{opt}$ = 3cm & 22.13 & 0.706 & \textbf{0.276} & 0.119\\
& $b_{opt}$ = 5cm & \textbf{22.36} & \textbf{0.707} & 0.281 & \textbf{0.117}\\
& $b_{opt}$ = 7cm & 22.21 & 0.705 & 0.284 & \textbf{0.117} \\
&$b_{opt}$ = 10cm & 22.21& 0.704& 0.284& \textbf{0.117} \\
\hline
\end{tabular}
}}

\caption{Performance comparison for different values of $b_{opt}$. We set the value for $i_{opt}$ as 300 for all experiments.}
\label{Table:ablation_loss_b_opt}
\end{table}

==> Tables_sup/ablation_loss_i_opt.tex <==
\begin{table}[h]{

\resizebox{\linewidth}{!}{%
\begin{tabular}{c|l|ccccc}
\hline

\multicolumn{2}{c|}{} & PSNR $\uparrow$& SSIM $\uparrow$ & LPIPS $\downarrow$ & RMSE $\downarrow$\\
\hline
\multicolumn{2}{c|}{Eikonal} & 20.82 & 0.610 & 0.391 & 0.226\\
\hline
\multirow{4}{*}{Ours}& $i_{opt}$ = 100 & 22.29& \textbf{0.714} & \textbf{0.281} & \textbf{0.112} \\
&$i_{opt}$ = 300 & \textbf{22.36} & 0.707 & \textbf{0.281} & 0.117\\
&$i_{opt}$ = 500 & 22.29& 0.704&0.283 & 0.119\\
&$i_{opt}$ = 1000 & 22.28 & 0.701 & 0.285 & 0.119\\
\hline
\end{tabular}
}}

\caption{Performance comparison for different values of $i_{opt}$ of our loss function. We set the value of $b_{opt}$ as 5cm for all experiments.}
\label{Table:ablation_loss_i_opt}
\end{table}

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec_sup/0_intro.tex <==
%This is a supplementary material for the paper, \emph{Stable Surface Regularization for Fast Few-Shot NeRF}. We will describe the comparisons for reconstruction results and geometry rendering and additional ablation studies of our loss function, hyperparameters $b_{opt}$ and $i_{opt}$, and comparisons with versions which are trained with the Eikonal loss with a larger loss weight.

This is supplementary material for the paper, \emph{Stable Surface Regularization for Fast Few-Shot NeRF}. We will provide descriptions of the comparisons for reconstruction results and geometry rendering, along with analyses of the hyperparameters $b_{opt}$ and $i_{opt}$ of our loss function. Additionally, we will compare our approach with versions trained using the Eikonal loss with a larger loss weight.

==> sec_sup/1_0_recon.tex <==
In this section, we compare our method with the previous works, \cite{roessle2022dense, deng2022depth, yu2022monosdf} and naive adaptation for \cite{sun2022direct} and the Eikonal loss~\cite{gropp2020implicit}, and ours by visualizing 3D mesh and rendered geometric prior in 4 scenes of ScanNet dataset~\cite{dai2017scannet} which is given by \cite{roessle2022dense}.

==> sec_sup/1_1_recon_results.tex <==
\noindent \textbf{Surface reconstruction.} \
The mesh visualizations for state-of-the-art works \cite{deng2022depth, roessle2022dense}, the naive approach of \cite{sun2022direct} and \cite{gropp2020implicit}, \cite{yu2022monosdf} and our method in the ScanNet dataset \cite{dai2017scannet} are displayed in Figure~\ref{Fig:sup_mesh}.

The visualized mesh reveals that previous works struggle to reconstruct the scene accurately, exhibiting issues such as ``floaters".
For approaches (a) DSNeRF~\cite{deng2022depth} and (b) DDPNeRF~\cite{roessle2022dense}, which utilize depth only for geometry supervision, they struggle to reconstruct the clear mesh due to the lack of geometry smoothing.
Also, approach (c), which employs Eikonal loss~\cite{gropp2020implicit} only, faces challenges with complex geometry and fails to reconstruct the scene.
As for MonoSDF~\cite{yu2022monosdf}, we believe that if there are few overlapping regions between images, many convergence points may occur, resulting in unstable optimization, and the simple loss function may not capture sufficient geometry information, leading to reconstruction failure.
However, our method overcomes these issues by using geometric smoothing and priors, and produces a clear mesh, as illustrated in (e).

\noindent \textbf{Neural Rendering.}
Figure~\ref{Fig:sup_mesh} presents the comparisons of rendering quality for RGB image and geometry prior, surface normal. Notably, approaches DSNeRF~\cite{deng2022depth} and DDPNeRF~\cite{roessle2022dense} do not incorporate surface normals, resulting in struggles with rendering surface normals accurately.
%DSNeRF~\cite{deng2022depth} and DDPNeRF~\cite{roessle2022dense} did not utilize surface normal, leading to struggles in rendering surface normal.
Conversely, approaches that utilize a surface loss, a naive adaptation of \cite{sun2022direct}, \cite{gropp2020implicit}, and MonoSDF~\cite{yu2022monosdf}, demonstrate significant improvements in the visual quality of surface normals.
%Conversely, approaches naive adaptation of \cite{sun2022direct} and \cite{gropp2020implicit}, and MonoSDF~\cite{yu2022monosdf} show that surface loss results in significant enhancement for visual quality of surface normal.
However, DDPNeRF~\cite{roessle2022dense} shows clearer visualization of color image than approaches that incorporate surface priors for certain parts, such as the T.V. in the last row, even when the surface normal is not captured accurately. It is worth noting that Eikonal loss~\cite{gropp2020implicit} may lead to unstable optimization in a few-view setup, resulting in a decrease in reconstructed quality for some scenes, as illustrated in the T.V. example in the last row of Figure~\ref{Fig:sup_mesh}.
In contrast, our approach produces clear geometry and rendering quality.

==> sec_sup/2_0_ablation.tex <==
%We provide the additional studies that we did not include in the manuscripts, which is about the hyperparameters of $b_{opt}$ and $i_{opt}$ which are used in the our loss and comparisons with models trained using the Eikonal loss with a larger loss weight.
%We conduct all evaluation for various $b_{opt}$ and $i_{opt}$ in the single scene, Scene0710 of the ScanNet dataset~\cite{dai2017scannet}. For this scene, the voxel resolution and voxel size is 289$\times$289$\times$193 and 2.5cm, respectively, for highest resolution grid to fit the GPU memory. It is also same for comparisons with another models.
We provide additional studies that were not included in the manuscript, focusing on the hyperparameters $b_{opt}$ and $i_{opt}$ used in our loss function, as well as comparisons with models trained using the Eikonal loss with a larger weight.
These evaluations are conducted exclusively on Scene0710 of the ScanNet dataset~\cite{dai2017scannet}, where we explore various combinations of $b_{opt}$ and $i_{opt}$, along with additional comparisons. In this scene, we use a voxel resolution of 289$\times$289$\times$193 and a voxel size of 2.5cm, tailored to fit the GPU memory constraints.

==> sec_sup/2_1_abl_recon_per_epoch.tex <==
We provide the additional studies for our loss functions for $b_{opt}$ and $i_{opt}$.
For the value $b_{opt}$, the size of voxel grid means that how much details will be considered. The smaller voxel grid, the more fine details be represented since the resolution will be increased. Especially, it is important to find best optimal value for $b_{opt}$ and the size of the voxel since how many we will smoooth geometry at final stage of annealing according to the size of the voxel which is determined GPU memory.
\input{Tables_sup/ablation_loss_b_opt}

Table~\ref{Table:ablation_loss_b_opt} depicts the performance dependency of our method on the hyperparameters $b_{opt}$.
The results demonstrate that our approach outperforms Eikonal loss~\cite{gropp2020implicit} for the any chosen values of both hyperparameters, as shown in Table~\ref{Table:ablation_loss_b_opt}.
As mentioned at initial of this section, it is important to choice how we choose the optimal value for $b$.
We empirically found that general $b_{opt}$ is between 2$\times$ to 3$\times$ of minimum size of the voxel.
For this scene, we choose 2 times value of minimum voxel grid 2.5cm, 5cm.
%For each scenes, we select $b_{opt}$ as a 3 times value for smallest size of the voxel grid. 
We did not use any adaptive strategy to determine $b_{opt}$, but we suggest that proposing an adaptive $b_{opt}$ algorithm could enhance our performance.

\input{Tables_sup/ablation_loss_i_opt}
We also observed the performance based on $i_{opt}$ in Table~\ref{Table:ablation_loss_i_opt}, which indicates how quickly the fine structure is recovered. 
As the table indicates, this parameter also affects the performance. 
We empirically found that the general value for $i_{opt}$ is 300. 
We believe that this is related to the scene's scale and complexity; for instance, a complex scene may require more time for the network to anneal geometry. 
Therefore, we suggest that an adaptive $i_{opt}$ strategy based on the scene's complexity or scale would be helpful in enhancing our approach's performance.

==> sec_sup/2_2_comparisons.tex <==
%In this section, we provide additional experiments with models trained using various weight for the Eikonal loss. There are 3 variations, the weight for the Eikonal loss 0.1 for (a), 1 for (b) and 10 for (c) as shown in Figure~\ref{Fig:sup_add_graph} and Figure~\ref{Fig:sup_add_viz}. all another weights are not in change. When we strongly press the eikonal loss weight, the weights are converged well as shown in (c) in Figure~\ref{Fig:sup_add_graph}. However, this means that it dives into local minima, as shown in the quantitative result shown in (c) in Figure~\ref{Fig:sup_add_viz}. Even its strong regularization for Eikonal loss, the effect seems hard to follow the effectiveness of our ASDF loss.
In this section, we provide additional experiments with models trained using various weights for the Eikonal loss. There are three variations: a weight of 0.1 for (a), 1 for (b), and 10 for (c) as shown in Figure~\ref{Fig:sup_add_graph} and Figure~\ref{Fig:sup_add_viz}. All other weights remain unchanged. Increasing the weight of the Eikonal loss significantly leads to its convergence, as shown in (c) in Figure~\ref{Fig:sup_add_graph}. However, this indicates that the model is trapped in local minima, as demonstrated by the quantitative results in (c) in Figure~\ref{Fig:sup_add_viz}. Despite its strong regularization of the Eikonal loss, its effectiveness appears to be limited compared to our ASDF loss.
